Visually Grounded Continual Language Learning with Selective Specialization

A desirable trait of an artificial agent acting in the visual world is to continually learn a sequence of language-informed tasks while striking a balance between sufficiently specializing in each task and building a generalized knowledge for transfer. Selective specialization, i.e., a careful selection of model components to specialize in each task, is a strategy to provide control over this trade-off. However, the design of selection strategies requires insights on the role of each model component in learning rather specialized or generalizable representations, which poses a gap in current research. Thus, our aim with this work is to provide an extensive analysis of selection strategies for visually grounded continual language learning. Due to the lack of suitable benchmarks for this purpose, we introduce two novel diagnostic datasets that provide enough control and flexibility for a thorough model analysis. We assess various heuristics for module specialization strategies as well as quantifiable measures for two different types of model architectures. Finally, we design conceptually simple approaches based on our analysis that outperform common continual learning baselines. Our results demonstrate the need for further efforts towards better aligning continual learning algorithms with the learning behaviors of individual model parts.

==> sections/9_some_thoughts.tex <==
\section{Some thoughts and former texts to be removed later}

\subsection{Differentiate from Mendez paper}

\paragraph{\textbf{What are limitations of the \citet{mendez_lifelong_2021} paper?}}

\begin{itemize}
    \item task IDs assumed during training and testing
    \item only applied to single-modality classification problems and simple architectures, thus scalability to bigger networks questionable $\to$ how to induce such compositional structures in vision-language architectures?
    \item Do not show to what extent assimilation and accommodation can reduce the need for newly seen data over time, even finally resulting in zero-shot capabilities of the model
    \item (Accommodation always follows assimilation $\to$ what if the model decides itself when to update the shared and when to update the task-specific parameters?)
    \item (structures and components are predefined $\to$ is there a way to find out suitable task-specific/task-agnostic parameters dynamically?)
    \item (number of learnable structs increases with every task $\to$ limited scalability)
\end{itemize}

\paragraph{\textbf{What is the outline of our work?}} Our aim is to extend the assimilation and accommodation paradigm as an inspiration to the work of \citet{mendez_lifelong_2021} towards more complex vision-language problems. First, we will determine whether the choices of structures/components as proposed in prior work, e.g., soft layer ordering, soft routing, and normalization scaling, are also applicable to vision-language models like transformers and FiLM. We will determine which parts/parameters of the model should be shared and which ones should specific to a task to make better use of the shared knowledge between tasks. Beyond that, we will  

\vspace{0.5cm}

\paragraph{\textbf{Why is it important?}}

Continual learning research overly focuses on preventing catastrophic forgetting, but has not made a substantial effort towards discovering explicit or implicit reusable knowledge to, on the one hand, accelerate forward transfer to new tasks and, on the other hand, restrict the updates of the model parts that solve subproblems shared across multiple tasks. Although there has been some initial research on separating the learning of shared model parts from the learning of task-specific parameters, the applicability and generalization of the insights gained in such works to more complex cross-modal interaction problems remains unsolved.

\vspace{0.5cm}

\paragraph{\textbf{What is the contribution of our work?}} We will propose two different diagnostic vision-language datasets (2D and 3D) with clearly defined semantic overlaps between tasks to enable a fine-grained analysis of the specialization and generalization behavior of different parts of the models. In addition, we propose an auxiliary learning scheme to predict the task IDs during continual learning phase to enable the model to automatically select the most suitable structure to be used during inference. 
%Finally, we will propose a mechanism that allows a model to do on-the-fly selection of task-specific and shared parameters that is more flexible with respect to the task at hand (?)

\subsection{Related Work}

\paragraph{Continual Lifelong Learning}

In a continual lifelong learning ({CLL}) scenario, a model is exposed to a sequence of tasks with the objective of having the model quickly adapt to the currently seen task while maintaining high performance on previous tasks. Several {CLL} methods have been proposed, which can be broadly categorized into the paradigms of regularization~\citep{kirkpatrick_ewc_2017,zenke_si_2017,li_lwf_2018,aljundi_mas_2018}, dynamic architectures~\cite{rusu_pnn_2016}, and rehearsal~\citep{lopez-paz_gem_2017,chaudhry_agem_2019}. The latter paradigm is also dominant for CLL problems in NLP, which applies to both text-only~\citep{de_masson_dautume_mbpa++_2019,sun_lamol_2020,wang_lifelong_fewrel_2019} and vision-language~\citep{hayes_remind_2020,jin_viscoll_2020,skantze_collie_2022} models. However, most CLL methods have been developed with an undue focus on overcoming catastrophic forgetting instead of identifying reusable knowledge.

\paragraph{Modeling Compositional Language}

We hypothesize that in a lifelong language learning scenario, captioning and reusing syntactic and semantic linguistic building blocks can make future learning more efficient while consolidating what has been learned in the past. Several attempts have been made to model the algebraic compositionality of language in NLP, vision-language, and grounded language tasks such as command-to-action translation~\citep{lake_scan_2018,liu_compositional_analytical_2020}, relational reasoning~\citep{sinha-clutrr-2019,dong_distilling_2020}, (visual) question answering~\citep{keysers_cfq_2020,bahdanau_closure_2019,bogin_compositional_vqa_2021}, visually grounded masked language modeling~\citep{jin_viscoll_2020,suris_expert_2020}, text-to-image retrieval~\citep{skantze_collie_2022}, and instruction following~\citep{ruis_gscan_2020,kuo-etal-2021-compositional-networks}. Recently, efforts have been made to inject compositional generalization into pretrained transformer models by means of tweaking model and training configurations \citep{csordas_devil_2021,ontanon_transformer_comp_2022} and data augmentation \citep{qiu_comp_augment_2022}.  

\paragraph{Compositional Language in Lifelong Learning}

We are aware of three works that investigate compositional language in a continual learning scenario:
\citet{li_clcl_2020} introduce an approach to decouple syntax and semantics of language input for instruction comprehension and machine translation tasks. 
%Their decoupling strategy is limited in that it relies on prior knowledge about the (rather simplistic) syntactic patterns of the input domain, leaving generalizability of their findings to other problem settings questionable. Moreover, this work builds exclusively on text comprehension, although it is widely argued that utterances and the meaning of language in context can only be constructed from multimodal perception~\citep{bisk-worldscopes-2020,vigliocco_language_multimodal_2014}. 
\citet{jin_viscoll_2020} explore the capabilities of LLL models to systematically generalize over adjective-noun combinations from an image-caption stream with gradually shifting task distributions. 
%However, the proposed scenario suffers from two limitations: First, the use of real images in this work impairs the assessment of compositional reasoning capabilities due to biases exploitable by models to circumvent reasoning~\citep{agrawal_vqa_bias_2016,zhang_vqa_bias_2016}. Second, the compositional phrases learnt by the models are restricted to a fixed syntactic structure, i.e. adjective-noun composites, bypassing systematic generalization at the level of complex tasks expressed in free-form natural language. 
\citet{skantze_collie_2022} propose a method to continually align the text embeddings of some pretrained vision-language encoder with its image embeddings via linear transformation. 
%Nevertheless, the learning scenario is fairly simplified, both with respect to single-object images as vision input and one or two word referential expressions as language input. Such facilitated learning conditions raise doubts about scalability and generalizability to more complex scenarios.   

However, none of the existing works give a thorough understanding about how the inductive bias of compositional language is related to a model's capabilities to learn more efficiently while overcoming forgetting in a lifelong learning scenario. 
%Moreover, the benchmarks and models in existing work are designed based on strong assumptions about the algebraic structure of the language input. 



\begin{itemize}
    \item At which modality fusion layers (early/late/intermediate) should we introduce task-specific parameters?
    \item Which modules of the networks naturally specialize on different tasks according several importance metrics from pruning research area?
    \item Which CL methods benefit from the distinction between shared and task-specific modules?
    \item ``Transformer Feed-Forward Layers Are Key-Value Memories'' (Geva et al.) What is the relation between their findings in the paper and the benefit of making certain feed-forward layers task-specific?
    \item Does the adaptation-consolidation scheme improve forward transfer to an extent that enables few-shot or even zero-shot capabilities?
    \item \textit{Is there a relationship between the number of shared parameters and the forward transfer?}
\end{itemize}

Goal: Learn more about the role of modules in vision-language models in terms of discovery of reusable knowledge, specialization, and avoiding interference. Show that with a careful analysis of which parameters should be specialized to a language-grounding task, the model only needs to be trained on all shared modules sparsely.
Related work: Adapters for continual learning (risk of task interference, limited adaptation capability, hand-engineered/role in transfer underexplored?), continual pruning strategies (do not inherently enable forward transfer, potential re-training and fine-tuning overhead).


\paragraph{\textbf{Problem setting, motivation}}

\begin{itemize}
    \item Continual learning research pays overly focus on catastrohpic forgetting
    \item Research should put more effort into discovery of reusable knowledge and potential sources interference
    \item Especially important for solving language grounding problems, as language is inherently combinatorial and compositional
    \item There is a need for fast, but robust vision-language grounding without forgetting, e.g. for autonomous agents in non-stationary settings that do not have unlimited amount of attempts to learn a new task
\end{itemize}

\paragraph{\textbf{How does our research fit in here?}}

\begin{itemize}
    \item Analyze for common vision-language models which parts of the model should be specialized and which ones should be shared across tasks to allow for transfer while preventing interference \textcolor{red}{differentiate from pruning methods}
    \item Show that, when used in a adaptation-consolidation (fast learning, slow learning) scheme, we can outperform established CL baselines with monolithic architectures while saving computation time (at the cost of an increase in memory), so this approach can potentially be used in bigger and pretrained models (future work?) \textcolor{red}{differentiate from architectural methods, e.g., adapters, why our scheme is better}
    \item Show that we can increase forward transfer to an extent that models are enabled one-/zero-shot performance on unseen combinations of inputs
\end{itemize}

\paragraph{\textbf{I: Finding the "right" modules to be specialized}}

\begin{itemize}
    \item early/late layers
    \item normalization scaling
    \item feedforward
    \item three importance metrics
    \item come up with task ID prediction scheme during testing and show that it does not lead to significantly degraded performance
\end{itemize}

\paragraph{\textbf{II: Adaptation-consolidation scheme}}

\begin{itemize}
    \item (go down the bio-inspired path here)
    \item combine with different baseline CL algorithms
    \item show that even outperforms CL algos for all-shared setting
    \item (analyze more in detail why it is better)
\end{itemize}

\paragraph{\textbf{III: Forward tranfer and one-/zero-shot}}

\begin{itemize}
    \item show that we can achieve zero-shot performance on unseen combinations of language primitives
    \item (with ablation study)
    \item even though we learn specialized parameters for different sets of language compositions, the rest of the model learns the shared underlying subproblem and can quickly put novel compositions into the shared context
    \item showcase that the superior performance is due to better knowledge reuse
\end{itemize}


Some thought: We propose a problem that is not classification and therefore does not allow for separated training of task-specific heads as an `easy' solution to the specialization question.
    

\clearpage



\iffalse

\begin{center}
\begin{table}[]
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c|c}
\textbf{CL Algo}                                                         & \textbf{Mode} & \textbf{LILAC-2D} & \textbf{LILAC-3D} \\ \hline
\multirow{3}{*}{ER}                                                      & Comp          & $\mathbf{ 63.98 \pm 2.8}\%$ & $ 87.05 \pm 0.0\%$ \\
                                                                         & Joint         & $ 62.64 \pm 2.1\%$ & $ \mathbf{89.98 \pm 0.0}\%$ \\
                                                                         & Mono          & $ 54.46 \pm 0.8\%$ & $ 84.78 \pm 10.0\%$\\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}EWC \\ (Online)\end{tabular}} & Comp          & $ \mathbf{56.20 \pm 3.5}\%$ & $ \mathbf{71.37 \pm 8.4}\%$ \\
                                                                         & Joint         & $ 52.44 \pm 1.7\%$ & $ 71.23 \pm 0.1\%$ \\
                                                                         & Mono          & $ 50.46 \pm 0.3\%$ & $ 70.78 \pm 0.6\%$ \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}EWC \\ (Memory)\end{tabular}} & Comp          & $ \mathbf{55.54 \pm 2.7}\%$ & $ \mathbf{73.97 \pm 4.7}\%$ \\
                                                                         & Joint         & $ 53.00 \pm 1.7\%$ & $ 67.74 \pm 5.0\%$ \\
                                                                         & Mono          & $ 50.09 \pm 0.7\%$ & $ 72.36 \pm 3.5\%$ \\ \hline
\multirow{3}{*}{Vanilla}                                                 & Comp          & $ \mathbf{56.22 \pm 2.3}\%$ & $ \mathbf{73.09 \pm 3.0}\%$ \\
                                                                         & Joint         & $ 52.64 \pm 0.6\%$ & $ 71.07 \pm 4.7\%$ \\
                                                                         & Mono          & $ 50.81 \pm 0.3\%$ & $ 70.50 \pm 1.9\%$                 
\end{tabular}
\caption{Average accuracy across sequentially seen tasks using feed-forward block of transformer layers as task-specific model components. Results are averaged across ten seeds. Standard error after $\pm$.}
\end{table}
\end{center}





\fi 
